The sharpness condition for constructing a finite element from a superspline

This paper addresses sharpness conditions for constructing $C^r$ conforming finite element spaces from a superspline spaces on general simplicial triangulations. We introduce the concept of extendability for the pre-element spaces, which encompasses both the superspline spaces and the finite element spaces. By examining the extendability condition for both types of spaces, we provide an answer to the conditions regarding the construction. A corollary of our results is that constructing $C^r$ conforming elements in $d$ dimensions generally requires an extra $C^{2^{s}r}$ continuity on $s$-codimensional simplices, and the polynomial degree is at least $(2^d r + 1)$.

==> fig/figure_k_2D.tex <==
\begin{tikzpicture}[scale=1.5]
    % 绘制卦限
    \filldraw[yellow,fill opacity=0.3] (-1,0) -- (0,-1) -- (0,0);
    \filldraw[blue,fill opacity=0.3] (-1,0) -- (-2,1) -- (-2,0);
    \filldraw[red,fill opacity=0.3] (1,0) -- (0,1) -- (0,0);

    \draw[line width=1pt,yellow!50!black] (-1,0) -- (0,-1) -- (0,0) -- cycle;
    \draw[line width=1pt,blue] (-1,0) -- (-2,1) -- (-2,0) -- cycle;
    \draw[line width=1pt,red] (1,0) -- (0,1) -- (0,0) -- cycle;

    %公共部分
    \fill[green] (-1, 0) circle(1.5pt);
    \fill[orange] (0,0) circle(1.5pt);

    % 添加文字
    % \draw[blue] (-5/3, 1/3) -- (-2, -1/2);
    % \node[below] at (-2, -1/2) {$K_{1}$};
    % \draw[red] (1/3, 1/3) -- (1, 1/2);
    % \node[right] at (1, 1/2) {$K_{0}$};
    % \draw[yellow!70!black] (-1/3, -1/3) -- (-1/2, 1/2);
    % \node[above] at (-1/2, 1/2) {$K$};
    \node[blue] at (-12/7, 2/7) {$K_{1}$};
    \node[red] at (2/7, 2/7) {$K_{0}$};
    \node[yellow!50!black] at (-2/7, -2/7) {$K$};
    \draw[green] (-1, 0) -- (-1, -1/2);
    \node[green, below] at (-1, -1/2) {$V_1$};
    \draw[orange] (0,0) -- (1/2, -1/2);
    \node[orange, below right] at (1/2, -1/2) {$V_0$};
\end{tikzpicture}

==> fig/figure_r_2D.tex <==
\begin{tikzpicture}[scale=1.5]
    % 绘制卦限
    \filldraw[yellow,fill opacity=0.3] (1,0) -- (0,-1) -- (0,0);
    \filldraw[blue,fill opacity=0.3] (-1,0) -- (0,-1) -- (0,0);
    \filldraw[red,fill opacity=0.3] (1,0) -- (0,1) -- (0,0);

    \draw[line width=1pt,yellow!50!black] (1,0) -- (0,-1) -- (0,0) -- cycle;
    \draw[line width=1pt,blue] (-1,0) -- (0,-1) -- (0,0) -- cycle;
    \draw[line width=1pt,red] (1,0) -- (0,1) -- (0,0) -- cycle;
    
    % 定义坐标系
    \draw (-1.5,0) -- (-1,0);
    \draw (0,-1.5) -- (0,-1);
    \draw[->,>=latex] (1,0) -- (1.5,0);
    \draw[->,>=latex] (0,1) -- (0,1.5);
    % 标记坐标轴
    \node[below] at (-1.5,0) {$-x_1$};
    \node[below] at (1.5,0) {$x_1$};
    \node[left] at (0,-1.5) {$-x_2$};
    \node[right] at (0,1.5) {$x_2$};

    %公共部分
    \draw[line width=2pt,green] (0,0) -- (0,-1);
    \draw[line width=2pt,orange] (0,0) -- (1,0);
    \fill[violet] (0,0) circle(1.5pt);

    % 添加文字
    % \draw[blue] (-1/3, -1/3) -- (-1, -1/2);
    % \node[left] at (-1, -1/2) {$K_{--}$};
    % \draw[red] (1/3, 1/3) -- (1, 1/2);
    % \node[above] at (1, 1/2) {$K_{++}$};
    % \draw[yellow!50!black] (1/3, -1/3) -- (1/2, -1);
    % \node[below] at (1/2, -1) {$K_{+-}$};
    % \node[color = blue] at (-1/3, -1/4) {$K_{--}$};
    % \node[color = red] at (1/3, 1/4) {$K_{++}$};
    % \node[color = yellow!50!black] at (1/3, -1/4) {$K_{+-}$};
    \node[blue] at (-1/3, -1/4) {$K_{--}$};
    \node[red] at (1/3, 1/4) {$K_{++}$};
    \node[yellow!50!black] at (1/3, -1/4) {$K_{+-}$};
    \draw[green] (0, -1/2) -- (-1/2, -1);
    \node[green, left] at (-1/2, -1) {$F_{2}$};
    \draw[orange] (1/2, 0) -- (1, -1/2);
    \node[orange, below] at (1, -1/2) {$F_{1}$};
    \draw[violet] (0, 0) -- (-1/2, 1/2);
    \node[violet, above left] at (-1/2, 1/2) {$V_{0}$};
\end{tikzpicture}

==> fig/figure_rd.tex <==
\begin{tikzpicture}[scale=1.5]
    % 绘制卦限
    \filldraw[blue,fill opacity=0.3] (-1,0,0) -- (0,-1,0) -- (0,0,-1);
    \filldraw[red,fill opacity=0.3] (1,0,0) -- (0,1,0) -- (0,0,1);
    
    \draw[line width=1pt,blue] (-1,0,0) -- (0,-1,0) -- (0,0,-1) -- cycle;
    \draw[line width=1pt,blue] (0,0,0) -- (-1,0,0);
    \draw[line width=1pt,blue] (0,0,0) -- (0,-1,0);
    \draw[line width=1pt,blue] (0,0,0)--(0,0,-1);
    
    \draw[line width=1pt,dashed,red] (0,0,0) -- (1,0,0);
    \draw[line width=1pt,dashed,red] (0,0,0) -- (0,1,0);
    \draw[line width=1pt,dashed,red] (0,0,0) -- (0,0,1);
    \draw[line width=1pt,red] (1,0,0) -- (0,1,0) -- (0,0,1) -- cycle;
    
    \fill[violet] (0,0,0) circle(1.5pt);
    
    % 定义坐标系
    \draw (-1.5,0,0) -- (-1,0,0);
    \draw (0,-1.5,0) -- (0,-1,0);
    \draw (0,0,-2) -- (0,0,-1);
    \draw[->,>=latex] (1,0,0) -- (1.5,0,0);
    \draw[->,>=latex] (0,1,0) -- (0,1.5,0);
    \draw[->,>=latex] (0,0,1) -- (0,0,2);
    
    % 标记坐标轴
    \node[below] at (-1.5,0,0) {$-x_1$};
    \node[below] at (1.5,0,0) {$x_1$};
    \node[left] at (0,-1.5,0) {$-x_2$};
    \node[right] at (0,1.5,0) {$x_2$};
    \node[above] at (0,0,-2) {$-x_3$};
    \node[below] at (0,0,2) {$x_3$};

    % 添加文字
    \draw[blue] (-0.25,-0.25,-0.25) -- (-1,0,-1);
    \node[blue, above left] at (-1,0,-1) {$K_{--}$};
    \draw[red] (0.25,0.25,0.25) -- (1,0,1);
    \node[red, below right] at (1,0,1) {$K_{++}$};
    \draw[violet] (0,0,0) -- (1,0,-1);
    \node[violet, right] at (1,0,-1) {$V_{0}$};
\end{tikzpicture}
\qquad
\begin{tikzpicture}[scale=1.5]
    % 绘制卦限
    \filldraw[yellow,fill opacity=0.3] (1,0,0) -- (0,1,0) -- (0,0,0);
    
    \draw[line width=1pt,dashed,yellow!50!black] (1,0,0) -- (0,0,-1);
    \draw[line width=1pt,dashed,yellow!50!black] (0,1,0) -- (0,0,-1);
    \draw[line width=1pt,yellow!50!black] (0,0,0) -- (1,0,0) -- (0,1,0);
    
    \draw[line width=2pt,dashed,green] (0,0,0)--(0,0,-1);
    \draw[line width=2pt,orange] (0,0,0) -- (0,1,0);
    
    % 定义坐标系
    \draw (-1.5,0,0) -- (0,0,0);
    \draw (0,-1.5,0) -- (0,0,0);
    \draw (0,0,-2) -- (0,0,-1);
    \draw[->,>=latex] (1,0,0) -- (1.5,0,0);
    \draw[->,>=latex] (0,1,0) -- (0,1.5,0);
    \draw[->,>=latex] (0,0,0) -- (0,0,2);
    
    % 标记坐标轴
    \node[below] at (-1.5,0,0) {$-x_1$};
    \node[below] at (1.5,0,0) {$x_1$};
    \node[left] at (0,-1.5,0) {$-x_2$};
    \node[right] at (0,1.5,0) {$x_2$};
    \node[above] at (0,0,-2) {$-x_3$};
    \node[below] at (0,0,2) {$x_3$};
    
    % 添加文字
    \draw[yellow!50!black] (0.25,0.25,-0.25) -- (1,0,-1);
    \node[yellow!50!black, above] at (1,0,-1) {$K_{+-}$};
    \draw[green] (0,0,-0.5) -- (0,-1,-1);
    \node[green, below] at (0,-1,-1) {$F_2$};
    \draw[orange] (0,0.5,0) -- (-1,0,-1);
    \node[orange, left] at (-1,0,-1) {$F_1$};
\end{tikzpicture}

==> fig/figure_rs.tex <==
\begin{tikzpicture}[scale=1.5]
    % 绘制卦限
    \filldraw[blue,fill opacity=0.3] (-1,0,0) -- (0,-1,0) -- (0,0,0);
    \filldraw[red,fill opacity=0.3] (1,0,0) -- (0,1,0) -- (0,0,1);
    
    \draw[line width=1pt,blue] (-1,0,0) -- (0,-1,0) -- (0,0,0) -- cycle;
    \draw[line width=1pt,blue] (-1,0,0) -- (0,0,1);
    \draw[line width=1pt,blue] (0,-1,0)--(0,0,1);
    
    \draw[line width=1pt,dashed,red] (0,0,0) -- (1,0,0);
    \draw[line width=1pt,dashed,red] (0,0,0) -- (0,1,0);
    \draw[line width=1pt,red] (1,0,0) -- (0,1,0) -- (0,0,1) -- cycle;
    
    \draw[line width=3pt,violet] (0,0,0) -- (0,0,1);
    
    % 定义坐标系
    \draw (-1.5,0,0) -- (-1,0,0);
    \draw (0,-1.5,0) -- (0,-1,0);
    \draw (0,0,-2) -- (0,0,0);
    \draw[->,>=latex] (1,0,0) -- (1.5,0,0);
    \draw[->,>=latex] (0,1,0) -- (0,1.5,0);
    \draw[->,>=latex] (0,0,1) -- (0,0,2);
    
    % 标记坐标轴
    \node[below] at (-1.5,0,0) {$-x_1$};
    \node[below] at (1.5,0,0) {$x_1$};
    \node[left] at (0,-1.5,0) {$-x_2$};
    \node[right] at (0,1.5,0) {$x_2$};
    \node[above] at (0,0,-2) {$-x_3$};
    \node[below] at (0,0,2) {$x_3$};

    % 添加文字
    \draw[blue] (-0.25,-0.25,0.25) -- (-1,0,-1);
    \node[blue, above] at (-1,0,-1) {$K_{--}$};
    \draw[red] (0.25,0.25,0.25) -- (1,0,-1);
    \node[red, right] at (1,0,-1) {$K_{++}$};
    \draw[violet] (0,0,0.5) -- (1,0,1);
    \node[violet, right] at (1,0,1) {$E$};
\end{tikzpicture}
\qquad
\begin{tikzpicture}[scale=1.5]
    % 绘制卦限
    \filldraw[green,fill opacity=0.3] (0,0,0) -- (0,0,1) -- (0,-1,0);
    \filldraw[yellow,fill opacity=0.3] (1,0,0) -- (0,0,0) -- (0,0,1);
    \filldraw[yellow,fill opacity=0.3] (1,0,0) -- (0,-1,0) -- (0,0,1);
    \filldraw[orange,fill opacity=0.3] (1,0,0) -- (0,0,0) -- (0,0,1);
    
    \draw[line width=1pt,yellow!50!black] (1,0,0) -- (0,-1,0);

    \draw[line width=2pt,green] (0,0,0) -- (0,0,1) -- (0,-1,0);
    \draw[line width=2pt,dashed,green] (0,0,0) -- (0,-1,0);
    \draw[line width=2pt,orange] (1,0,0) -- (0,0,0) -- (0,0,1) -- cycle;
    
    % 定义坐标系
    \draw (-1.5,0,0) -- (0,0,0);
    \draw (0,-1.5,0) -- (0,-1,0);
    \draw (0,0,-2) -- (0,0,0);
    \draw[->,>=latex] (1,0,0) -- (1.5,0,0);
    \draw[->,>=latex] (0,0,0) -- (0,1.5,0);
    \draw[->,>=latex] (0,0,1) -- (0,0,2);
    
    % 标记坐标轴
    \node[below] at (-1.5,0,0) {$-x_1$};
    \node[below] at (1.5,0,0) {$x_1$};
    \node[left] at (0,-1.5,0) {$-x_2$};
    \node[right] at (0,1.5,0) {$x_2$};
    \node[above] at (0,0,-2) {$-x_3$};
    \node[below] at (0,0,2) {$x_3$};
    
    % 添加文字
    \draw[yellow!50!black] (0.25,-0.25,0.25) -- (1,-1,0);
    \node[yellow!50!black, below] at (1,-1,0) {$K_{+-}$};
    \draw[green] (0,-1/3,1/3) -- (-1,0,-1);
    \node[green, above] at (-1,0,-1) {$F_2$};
    \draw[orange] (1/3,0,1/3) -- (1,0,-1);
    \node[orange, above] at (1,0,-1) {$F_1$};
\end{tikzpicture}
